Leveraging Neural Network Gradients within Trajectory Optimization for Proactive Human-Robot Interactions

To achieve seamless human-robot interactions, robots need to intimately reason about complex interaction dynamics and future human behaviors within their motion planning process. However, there is a disconnect between state-of-the-art neural network-based human behavior models and robot motion planners -- either the behavior models are limited in their consideration of downstream planning or a simplified behavior model is used to ensure tractability of the planning problem. In this work, we present a framework that fuses together the interpretability and flexibility of trajectory optimization (TO) with the predictive power of state-of-the-art human trajectory prediction models. In particular, we leverage gradient information from data-driven prediction models to explicitly reason about human-robot interaction dynamics within a gradient-based TO problem. We demonstrate the efficacy of our approach in a multi-agent scenario whereby a robot is required to safely and efficiently navigate through a crowd of up to ten pedestrians. We compare against a variety of planning methods, and show that by explicitly accounting for interaction dynamics within the planner, our method offers safer and more efficient behaviors, even yielding proactive and nuanced behaviors such as waiting for a pedestrian to pass before moving.

==> relatedwork.tex <==
\section{Related Work}\label{sec:related_work}
% One approach is model-based: decouple environmental modeling with planning. learn a model that describes the environment, in this case, interaction dynamics, and design a planner that leverages the prediction (Dorsa, Haruki, Schmerling). 
We review robot planning under uncertainty frameworks with a focus on planning in interactive settings characterized by multimodal uncertainty.
Conceptually, robot motion planning under uncertainty involves designing optimal strategies for a robot despite an incomplete knowledge of how exactly the robot and/or environment may behave. As such, robot motion planning under uncertainty can be formalized as a \ac{POMDP} \cite{KaelblingLittmanEtAl1998}, where the state of the system evolves according to a controlled Markov chain, the state is only partially observed, and one seeks to design a policy that maps state probability distributions to actions.
Despite theoretical and practical successes of \ac{POMDP} theory \cite{KaelblingLittmanEtAl1998,KurniawatiHsuEtAl2008,SomaniYeEtAl2013,KurniawatiDuEtAl2010,SunbergKochenderfer2018,BaiCaiEtAl2015}, online computation of a robot policy is extremely computationally intensive, leverages simplifying modeling assumptions (e.g., discretizing the action space), suffers from the curse of dimensionality, and has only been successfully applied to very small and low-dimensional state and action spaces. Thus leading the \ac{POMDP} formulation to be intractable for highly interactive multi-agent settings where the uncertainty, stemming from future human behaviors, is extremely complex and coupled.  

An alternative and widely adopted approach is to compute open-loop trajectories (instead of a closed-loop control policy) in a receding horizon fashion. By replanning frequently, the robot is able to update its plans to adjust for changes introduced by uncertainty in the system. 
% Common approaches to computing open-loop trajectories in uncertain environment include sampling-based motion planning (e.g., rapidly-exploring random trees (RRT) \cite{LaValleKuffner2001}), search-based methods (e.g., search over motion primitives \cite{SchmerlingLeungEtAl2018}) and trajectory optimization (TO) which casts the problem as a constrained optimization problem (e.g., \cite{BlackmoreOnoEtAl2010,BonalliCauligiEtAl2019}).
\ac{TO} is a popular open-loop method that strives to minimize a planning objective, such as control effort and travel time, subject to dynamic, state, and control constraints. 
% Naturally, the optimization problem becomes more difficult to solve when non-linear and non-convex elements are introduced, such through the objective function or dynamics.
% Finding Locally Optimal, Collision-Free Trajectories with Sequential Convex Optimization paper
\ac{TO} has been extensively used in many real-world settings that require a fast replanning frequency \cite{SpielbergBrownEtAl2019,Winkler2018}. Advantages of using \ac{TO} include the transparency and interpretability of the algorithm, ability to leverage highly-optimized off-the-shelf solvers for fast run-time, adaptability to new environments, and flexibility for a designer to specify desired behaviors at run-time.
% However, to ensure computational tractability and fast solve-times, the TO problem relies on tractable mathematical representations such as Gaussian noise on the system, or convexity in the optimization formulation. 
However, using \ac{TO} to plan for trajectories that enable a robot to interact with humans is computationally challenging because the uncertainty in human behavior is multimodal (i.e., there are possibly multiple distinct behaviors) and highly coupled (i.e., a human's behavior may depend on current and possible future actions of a robot).
%, all elements that make the \ac{TO} problem computationally difficult to solve.

% such methods assume that the environment, uncertain is mathematically well characterized (e.g., gaussian uncertainty on the position of an obstacle, gaussian white noise on the system dynamics), and thus are limited when dealing with uncertainty characteristic to human-robot interactions, that is, multimodal uncertainty that may be conditioned on past interactions and future robot actions.

Recent advances in deep neural networks and the availability of large datasets have enabled highly expressive human behavior prediction models which can learn arbitrarily complex (i.e., multimodal) probability distributions conditioned on many types of variables such as past interactions, images, maps, agent-type, etc. (e.g., \cite{SalzmannIvanovicEtAl2020,GuptaJohnsonEtAl2018,KosarajuSadeghianEtAl2019}). Despite their success in producing highly-accurate human behavior predictions,
%and ability to offer relatively high accuracy in human behavior predictions, 
a majority of these models remain disconnected from downstream planning and control. Only recently have behavior prediction models been made cognizant of downstream planning and control algorithms, however the chosen algorithms are usually tailored to a particular prediction model or treated as future work \cite{IvanovicElhafsiEtAl2020,ZhaoGaoEtAl2020}.
Considering that many deep learned prediction models produce samples of future human trajectories, a robot planner incorporating this type of output structure may rely on Monte Carlo sampling to estimate the interaction-dependent cost of selecting a particular control sequence, searching for the control sequence that corresponds to the lowest expected cost \cite{SchmerlingLeungEtAl2018,NishimuraIvanovicEtAl2020}. While search-based methods show promising results in real-world experiments, the quality of the search is limited by the replanning rate (usually $\sim$10Hz for rapidly-evolving interactive environments) thereby potentially missing rare yet catastrophic outcomes. Further, nuanced behaviors may be precluded by the discrete nature of the search and safety is only incentivized via the objective function rather than treated as a constraint.

Ensuring safety for human-robot interactions is paramount, yet challenging due to the uncertainty in human behaviors, especially since interactions inherently require the robot and humans to operate in close-proximity with each other.
Safety can be incentivized via the planning cost \cite{SchmerlingLeungEtAl2018, SadighSastryEtAl2016c} but it competes with other planning objectives, or via chance constraints \cite{LewBonalliECC2020} but assumes  unimodal/Gaussian uncertainty. Alternatively, safety can be enforced by only selecting plans that avoid the forward reachable set of other agents \cite{AlthoffDolan2011,LorenzettiChenEtAl2018}, or planning robust trajectory tubes that provide a buffer between the robot and obstacles \cite{MajumdarTedrake2017,SinghMajumdarEtAl2017,Fridovich-KeilHerbertEtAl2018}. However, many of these methods account for uncertainty in the robot's dynamics and/or static obstacles, and not for the coupling between the robot and humans' dynamics. 
To this end, we leverage \ac{HJ} backward reachability analysis \cite{MitchellBayenEtAl2005}, a formal verification tool for guaranteeing closed-loop safety of a system subjected to disturbances by the environment. Notably, \ac{HJ} reachability is independent of the prediction or planning model used, making it a useful and flexible tool in ensuring safety for a wide range of applications (e.g., \cite{FisacAkametaluEtAl2018,LeungSchmerlingEtAl2019,BajcsyBansalEtAl2019,WangLeungEtAl2020}).

In contrast to deep learned human behavior prediction models, \cite{SadighSastryEtAl2016c} uses handcrafted interpretable features to learn an analytic representation of a human's internal reward function using Inverse Reinforcement Learning \cite{ZiebartMaasEtAl2008,LevineKoltun2012}. As such, gradient information from the human behavior model is directly incorporated into the trajectory optimization formulation and off-the-shelf gradient-based solvers can be used. By tightly coupling modeling and control, the robot was able to effectively leverage the human behavior model within the optimization problem and produce human-interpretable behaviors without relying on hand-coded heuristics. We strive to follow this paradigm of using gradient information from the human behavior prediction model directly into the \ac{TO} problem. In particular, we aim to develop a paradigm that enables the use of complex deep neural network models within the \ac{TO} formulation since many of these models are state-of-the-art in human behavior (trajectory) prediction (e.g., see the nuScenes \cite{CaesarBankitiEtAl2019} prediction challenge leaderboard).
